A Dynamical Perspective on Point Cloud Registration

We provide a dynamical perspective on the classical problem of 3D point cloud registration with correspondences. A point cloud is considered as a rigid body consisting of particles. The problem of registering two point clouds is formulated as a dynamical system, where the dynamic model point cloud translates and rotates in a viscous environment towards the static scene point cloud, under forces and torques induced by virtual springs placed between each pair of corresponding points. We first show that the potential energy of the system recovers the objective function of the maximum likelihood estimation. We then adopt Lyapunov analysis, particularly the invariant set theorem, to analyze the rigid body dynamics and show that the system globally asymptotically tends towards the set of equilibrium points, where the globally optimal registration solution lies in. We conjecture that, besides the globally optimal equilibrium point, the system has either three or infinite "spurious" equilibrium points, and these spurious equilibria are all locally unstable. The case of three spurious equilibria corresponds to generic shape of the point cloud, while the case of infinite spurious equilibria happens when the point cloud exhibits symmetry. Therefore, simulating the dynamics with random perturbations guarantees to obtain the globally optimal registration solution. Numerical experiments support our analysis and conjecture.

==> outlier-free-registration.tex <==
%!TEX root = main.tex
\section{Outlier-free Registration}
The given points $\vxx_i$ and $\vy_i$ are measured in the same coordinate system. Assume all the points in both point clouds have equal mass $m=1$, so that the center of mass (CM) of $\calX$ is located at $\bar{\vxx} = (\sum_{i=1}^N \vxx_i) / N$ and the CM of $\calY$ is located at $\bar{\vy} = (\sum_{i=1}^N \vy_i) / N$.  Without loss of generality, suppose the scene cloud $\calY$ is already centered at zero,~\ie~$\bar{\vy} = \zero$,\footnote{Otherwise, we can shift every point by $\bar{\vy}$: $\vy_i \leftarrow \vy_i - \bar{\vy},\vxx_i \leftarrow \vxx_i - \bar{\vy}$.} and we attach a fixed global coordinate frame $Y$ at the CM of $\calY$. Further, we assume that each point $\vy_i$ is fixed and cannot move. 

For $\calX$, since it is an dynamic object, we attach a moving coordinate frame $X$ to its CM. At time $t \geq 0$, we let $\vxx_i^Y(t) \in \Real{d}$ (resp. $\vv_i^Y(t) \doteq \dvxx_i^Y$) be the position (resp. velocity) of the $i$-th point in frame $Y$; $\xcom^Y(t) \in \Real{d}$ (resp. $\xcomv^Y(t) \doteq \dxcom^Y$) be the position (resp. velocity) of the CM of point cloud $\calX$ in the fixed coordinate frame $Y$; let $\MR(t) \doteq \MR^Y_X(t) \in \SOthree$ be the rotation matrix that describes the relative attitude between frame $X$ and $Y$; let $\xangv^X(t) \in \Real{3}$ be the angular velocity of point cloud $\calX$ \wrt its CM in frame $X$. Then the tuple $(\xcom^Y, \xcomv^Y, \MR, \xangv^X)$ fully describes the state of point cloud $\calX$. With slight abuse of notation, we consider the following initial condition:
\bea
\xcom^Y(0) = \xcom = \frac{\sumallpoints \vxx_i}{N}, \quad \xcomv^Y(0) = \zero, \quad \MR(0) = \eye, \quad \xangv^X(0) = \zero,
\eea
which basically means that point cloud $\calX$ is at rest position and frame $X$ is axis-aligned with frame $Y$. In addition, we let $\xref_i \doteq \vxx_i - \xcom$ be the relative position of the $i$-th point \wrt the CM. Since we assume $\calX$ is a rigid body, we have $\vxx_i^X(t) = \xref_i, \forall t \geq 0$, and $\vxx_i^X, \vxx_i^Y$ are related through:
\bea
\vxx_i^Y = \MR \vxx_i^X + \xcom^Y.
\eea

From the Newton-Euler equation, the dynamics of $\calX$ reads:
\bea
\begin{cases}
\vf^Y = M \xcoma^Y \\
\vtau^X = \MJ \xanga^X + \xangv^X \times \MJ \xangv^X \\
\dMR = \MR \hatmap{\xangv^X} \\
\dxcom^Y = \xcomv^Y
\end{cases},
\eea
where $\xcoma^Y \doteq \dot{\xcomv}^Y$ denotes the translational acceleration of the CM of $\calX$ in frame $Y$, $\xanga^X \doteq \dot{\xangv}^X$ denotes the rotational acceleration of $\calX$ \wrt its CM, $M = Nm$ is the total mass of $\calX$, $\MJ \in \Real{d \times d}$ is the inertia matrix of $\calX$ \wrt the CM, $\vf^Y$ is the sum of all external forces in frame $Y$ and $\vtau^X$ is the sum of all external torques \wrt to the CM in frame $X$. Now we derive $\vf^Y$ and $\vtau^X$.

{\bf Force $\vf^Y$.} Assume the coefficient of the virtual spring between $\vxx_i$ and $\vy_i$ is $k_i>0$, and cloud $\calX$ is moving in a viscous fluid with damping coefficient $\mu>0$, then the force acting on each point $\vxx_i$, expressed in frame $Y$, is:
\bea
\vf_i^Y = k_i (\vy_i - \vxx_i^Y) - \mu \vv_i^Y = k_i (\vy_i - \MR \xref_i - \xcom^Y) - \mu (\MR(\xangv^X \times \xref_i) + \xcomv^Y), \label{eq:forcepointiY}
\eea
and hence the total force is:
\bea
\vf^Y = \sumallpoints \vf_i^Y = \sumallpoints k_i \left( \vy_i - \MR \xref_i - \xcom^Y  \right) - \mu N \xcomv^Y,
\eea
where we have used:
\bea
\sumallpoints \mu \MR (\xangv^X \times \xref_i ) = \sumallpoints \mu \MR \hatmap{\xangv^X} \xref_i = \mu\MR\hatmap{\xangv^X} \left( \sumallpoints \xref_i \right) = \zero,
\eea
due to the definition of $\xref_i = \vxx_i - \xcom$. 

{\bf Torque $\vtau^X$.} From the expression of $\vf_i^Y$ in eq.~\eqref{eq:forcepointiY}, we can find the expression of $\vf_i^X$:
\bea
\vf_i^X = \MR\tran \vf_i^Y = k_i \left( \MR\tran \vy_i - \xref_i - \MR\tran \xcom^Y \right) - \mu \left( \xangv^X \times \xref_i + \MR\tran \xcomv^Y \right).
\eea
Hence, we can compute the total torque:
\bea
\vtau^X = \sumallpoints \xref_i \times \vf_i^X = \sumallpoints \left( k_i \hatmap{\xref_i} \MR\tran \left( \vy_i - \xcom^Y \right) - \mu \hatmap{\xref_i}\hatmap{\xangv^X}\xref_i \right).
\eea
{\bf Equilibrium of the system.} With the expressions of the total force and torque, we can analyze the equilibrium point of the system. The equilibrium point must satisfies:
\bea
\xcoma^Y  = \zero, \quad \xanga^X = \zero, \quad \dMR = \zero, \quad \xcomv^Y = \zero,
\eea
which implies that:
\bea
\begin{cases}
\vf^Y = \sumallpoints \vf_i^Y = \sumallpoints k_i \left( \vy_i - \MR \xref_i - \xcom^Y  \right) - \mu N \xcomv^Y = \zero \\
\vtau^X = \sumallpoints \left( k_i \hatmap{\xref_i} \MR\tran \left( \vy_i - \xcom^Y \right) - \mu \hatmap{\xref_i}\hatmap{\xangv^X}\xref_i \right) = \zero \\
\xcomv^Y = \zero \\
\xangv^X = \zero
\end{cases}
\eea
and therefore:
\bea
\begin{cases}
\sumallpoints k_i \left( \vy_i - \MR \xref_i - \xcom^Y  \right) = \zero \\
 \sumallpoints  k_i \hatmap{\xref_i} \MR\tran \left( \vy_i - \xcom^Y \right) = \zero
\end{cases}.
\eea

{\bf Stability Analysis.} Consider the total energy of the system as the Lyapunov function:
\bea
& V = \displaystyle \sumallpoints \half m \left\| \vv_i^Y \right\|^2 + \sumallpoints \half k_i \left\| \vy_i - \MR \xref_i - \xcom^Y \right\|^2 \\
& = \displaystyle \underbrace{ \frac{M}{2} \left\| \xcomv^Y \right\|^2 + \half \left( \xangv^X \right)\tran \MJ \xangv^X}_{V_k} + \underbrace{ \sumallpoints \half k_i \left\| \vy_i - \MR \xref_i - \xcom^Y \right\|^2 }_{V_p}
\eea
where $V_k$ is the kinetic energy and $V_p$ is the potential energy. To derive the time derivative of $V$, we first compute the time derivative of $V_k$:
\bea
& \dV_k = \left( \xcomv^Y \right)\tran \left( M \xcoma^Y \right) + \left( \xangv^X \right)\tran \left(\MJ \xanga^X \right) \\
& = \left( \xcomv^Y \right)\tran \vf^Y + \left( \xangv^X \right)\tran \left( \vtau^X - \xangv^X \times \MJ \xangv^X \right) \\
& = \left( \xcomv^Y \right)\tran \left( \sum_i k_i \left( \vy_i - \MR \xref_i - \xcom^Y  \right) - \mu N \xcomv^Y \right) +  \\
& \left( \xangv^X \right)\tran \left( \sum_i \left( k_i \hatmap{\xref_i} \MR\tran \left( \vy_i - \xcom^Y \right) - \mu \hatmap{\xref_i}\hatmap{\xangv^X}\xref_i \right) \right) \\
& = - \mu N \| \xcomv^Y \|^2 - \mu \left( \xangv^X \right) \tran \frac{\MJ}{m} \left( \xangv^X \right) + \\
& \sum_i k_i \left( \xcomv^Y \right)\tran \left( \vy_i - \MR \xref_i - \xcom^Y  \right) + 
 \sum_i k_i \left(\MR \hatmap{\xangv^X} \xref_i \right)\tran \left( \vy_i - \xcom^Y \right),
\eea
and then we compute the time derivative of $V_p$:
\bea
\dV_p = \sum_i k_i \left( \vy_i - \MR \xref_i - \xcom^Y \right)\tran\left( - \MR\hatmap{\xangv^X} \xref_i - \xcomv^Y \right),
\eea
and we see that after cancellation of terms, $\dV$ is:
\bea
\dV = - \mu N \| \xcomv^Y \|^2 - \mu \left( \xangv^X \right) \tran \frac{\MJ}{m} \left( \xangv^X \right) =- \mu \sumallpoints \left\| \vv_i^Y \right\|^2,
\eea
which is indeed the energy dissipation from viscous damping. The invariant set theorem tells us the system will tend to the largest invariant set, which is the unique equilibrium point. 

\red{\bf Is the system contracting?}



==> problem_statement.tex <==
%!TEX root = main.tex
\section{Problem Statement}
Given two point clouds $\calX = \{ \vxx_i \}_{i=1}^N$ and $\calY = \{ \vy_i \}_{i=1}^N,\vxx_i,\vy_i \in \Real{d}$ ($d=2,3$), with putative correspondences $\vxx_i \leftrightarrow \vy_i$ (\eg~obtained from hand-crafted or deep-learned feature matching), \emph{point cloud registration} seeks to find the best \emph{rigid transformation} $(\MR \in \SOd,\vt \in \Real{d})$\footnote{$\SOd \doteq \{ \MR \in \Real{d\times d}: \MR\tran\MR = \MR\MR\tran = \eye_d, \det(\MR) = +1 \}$, where $\eye_d$ is the identity matrix of size $d$.} to align $\calX$ to $\calY$ ($\calX$ is called the \emph{model}, while $\calY$ is called the \emph{scene}). When all the correspondences are correct,~\ie~\emph{inliers}, the problem admits a closed-form solution due to Horn~\cite{Horn87josa}. Recent work by Yang~\etal~shows that the problem can be solved with \emph{global optimality certificate} using semidefinite relaxations~\cite{Yang20arxiv-teaser,Yang19rss-teaser}.

In this work, we propose to solve point cloud registration by modeling the alignment as a \emph{dynamical system} where the \emph{static and fixed} scene $\calY$ exerts \emph{virtual mechanical forces} to attract and move the model $\calX$. In particular, as illustrated in Fig.~\ref{fig:alignment-dynamics}, both $\calX$ and $\calY$ are considered as \emph{rigid bodies} with points in a global coordinate system $G$, with $\calY$ fixed such that it is always static. We place virtual springs and dampers between each pair of points $(\vxx_i,\vy_i)$ so that $\vy_i$ exerts an attractive force $\vf_i$ on $\vxx_i$. Under all pairwise forces $\vf_i$, $\calX$ rotates and translates according to the law of rigid body dynamics. By posing the registration problem as a dynamical system, we hope to leverage tools in control theory, in particular, Lyapunov stability theory and contraction theory, to study the following questions:
\begin{enumerate}
	\item Can we design the virtual (nonlinear) springs and dampers such that the dynamical system has a unique equilibrium point that is \emph{globally asymptotically/exponentially stable}, or such that the dynamical system is \emph{globally contracting}?
	\item Can we answer question 1 in the presence of \emph{outliers}?
	\item Can we answer question 1 when no correspondences are available? 
\end{enumerate}
The answers to the questions above will help analyze and design algorithms for solving point cloud registration (one can simply run the dynamics, the rigid transformation can be obtained using Horn's method~\cite{Horn87josa} at convergence).

{\bf Novelty:} Physics-based point cloud registration has been recently proposed in~\cite{Golyanik16CVPR-gravitationalRegistration,Jauer18PAMI-physicsBasedRegistration} as a local method to solve point cloud registration. Our main contributions are twofold: (i) we adopt virtual forces generated from virtual springs and dampers, while~\cite{Golyanik16CVPR-gravitationalRegistration,Jauer18PAMI-physicsBasedRegistration} use virtual forces generated by Gravitational forces and Coulomb forces, both of which suffer from singularities when the distance between $\vxx_i$ and $\vy_i$ is zero; (ii) no convergence analysis are known in previous works, while we leverage control theory to analyze the stability and contraction properties of the dynamical system, which directly translates to convergence analysis; (iii) allowing nonlinear springs and dampers may give rise to novel algorithms with global convergence guarantees.

\input{fig-alignment_dynamics}

==> robust-registration.tex <==
%!TEX root = main.tex
\section{Robust Registration}
\red{\bf L-1 Loss, Huber Loss, Geman-McClure Loss, and nonlinear springs.}


We want the total energy of the system to be:
\bea
V = \sumallpoints \min\left( \frac{1}{\beta_i^2} \left\| \vy_i - \MR \xref_i - \xcom^Y \right\|^2, \barcsq  \right) + \sumallpoints \half m \left\| \vv_i^Y \right\|^2,
\eea
which implies that the potential energy of each virtual spring saturates at $\barcsq$. Let the spring coefficient be:
\bea
k_i = \begin{cases}
\frac{2}{\beta_i^2} & \text{if } \left\| \vy_i - \MR \xref_i - \xcom^Y \right\|^2 \leq \barcsq \beta_i^2 \\
0 & \text{otherwise}
\end{cases}
\eea
This creates the issue that when $\calX$ is far away from $\calY$, there is zero spring force and $\calX$ keeps stationary.

\bea
\min_{\substack{c_k \geq 0,\vt \in \Real{2},\\ \MR \in \SOthree}} \sum_{i=1}^N \min\left( \left\| \vz_i - \Pi\MR \left( \sum_{k=1}^K c_k \MB_{ki} \right) -\vt \right\|^2, \barcsq\right) + \alpha \sum_{k=1}^K c_k
\eea

\bea
\min_{\substack{c_k \geq 0,\vt \in \Real{2},\\ \MR \in \SOthree}} \sum_{i=1}^N w_i \left\| \vz_i - \Pi\MR \left( \sum_{k=1}^K c_k \MB_{ki} \right) -\vt \right\|^2  + \Phi^\mu (w_i) + \alpha \sum_{k=1}^K c_k
\eea
